A robust dynamic mode decomposition methodology for an airfoil undergoing transonic shock buffet

Dynamic mode decomposition (DMD) is a data-driven technique widely used to analyze and model fluid problems including transonic buffet flows. Despite its strengths, DMD is known to suffer from sensitivities to the selected settings and the characteristics of the employed data. In this work, we closely examine the aforementioned sensitivities, identify possible pitfalls, and provide best practices to robustly perform DMD on a flow exhibiting transonic shock buffet. Specifically, we assess various DMD variants and test their sensitivity to the POD rank truncation and the sampling rate. A critical enabler to our analysis is a new presentation of the DMD algorithm as a modular framework consisting of five distinct steps. The tests also highlight the existing dangers of aliasing, when the sampling rate is too low. Finally, a list of practical recommendations and guidelines on how to accurately and robustly perform DMD on a transonic buffet flow is provided.

==> datasets.tex <==

The current investigations are based on numerical simulation data.
Within the project, multiple two- and three-dimensional simulations with different mesh resolutions and settings were conducted and validated \cite{weiner2022}.
%In this section, we present two selected three-dimensional simulations.
However, the current DMD analysis relies only on one three-dimensional numerical simulation setup.
In this section, we briefly describe the numerical approach, the validation process, and the data acquisition.
For more details, the reader is referred to Weiner and Semaan \cite{weiner2022}.

\subsection{Simulation approach}
% solver
The simulations are performed using the \textit{rhoCentralFoam} solver from the \textit{OpenFOAM-v2012}\footnote{\url{https://www.openfoam.com/}} library.
\textit{OpenFOAM} implements a finite volume approach for unstructured meshes with a cell-centered, co-located variable arrangement. 
Face fluxes are reconstructed based on the two neighboring cell-centered values of each face. 
\textit{rhoCentralFoam} solves the conservation equations for mass, momentum, and energy by operator splitting \cite{greenshields2010}. 
In the predictor step, the convection of conserved quantities, i.e., mass density, momentum density, and energy density, are computed explicitly. 
In the corrector step for momentum and energy, the diffusive terms are discretized and solved implicitly for the primitive variables, i.e., energy and velocity. 
The convective transport is computed based on the interpolation scheme by Kurganov et al. \cite{kurganov2001}. 
To interpolate the cell-centered values of the conserved variables to the faces, van Leer's limiter \cite{vanleer1974} is employed. 
Linear interpolation is used for all remaining face interpolations.

% turbulence modeling
The solver supports generic RANS, LES, or hybrid RANS-LES approaches. 
Attempts to predict transonic buffet with standard SA and $k$-$\omega$-SST RANS method at a critical angle of attack were not successful \cite{weiner2022}.
The solution converged to a steady state, which is a commonly-reported problem when employing RANS \cite{weiner2022,zimmermann2018,poplingher2019}.
Instead of modifying model constants or increasing the angle of attack to trigger the buffet, we resort to hybrid SA-IDDES simulations.
Our SA-IDDES implementation is based on the work by Gritskevich et al. \cite{gritskevich2012}. 
As detailed in \cite{weiner2022}, the IDDES simulations are capable of capturing the flow physics including the buffet phenomenon.

% airfoil geometry and mesh
The airfoil geometry is a simple subsonic NACA-0012 with a blunt trailing edge of height $2.5\times 10^{-3} c$, where $c$ denotes the chord length.
The choice for the popular NACA-0012 is motivated by our desire to use a public domain geometry for which experimental data are available.
% Three numerical meshes are tested.
The airfoil geometry along with the computational mesh is presented in figure \ref{fig:mesh}.
% Mesh refinement is conducted such that the aspect ratio of cells near the surface remains approximately constant.
% Table \ref{tab:meshes} show the overall number of control volumes and the wall-normal resolution in terms of inner wall units $y^+=\frac{y u_\tau}{\nu}$ for different refinement levels,
% where $u_\tau$ is the friction velocity and $\nu$ is the kinematic viscosity.
% The employed mesh for the current analysis 
The block-structured C-type mesh is generated with the \textit{blockMesh} utility. 
It consists of a total of $N_\mathrm{cells}\approx 4.9\times 10^6$ cells, 
and a wall-normal resolution of $y^+=\frac{y u_\tau}{\nu} =3.73$,
where $u_\tau$ is the friction velocity and $\nu$ is the kinematic viscosity.
Considering the airfoil's nose as the origin, the lower, upper, and upstream boundaries are located at a distance of $10c$, 
whereas the downstream boundary is $30c$ away. 
The mesh has a spanwise width of $0.2c$, and most surface elements have an aspect ratio close to unity.
% To have a quick and computationally cheap way of testing various meshing strategies and resolutions, we also performed 2D simulations.
% The 2D meshes are identical to their 3D counterparts but have only one cell in the spanwise direction.

% \begin{table}[hbt!]
% \caption{\label{tab:meshes} Parameters of 2D mesh dependency study; $y^+$ denotes the inner wall normal unit averaged over the airfoil at $\alpha = 2^\circ$; $N_{cells}$ is the number of control volumes.}
% \centering
% \begin{tabular}{r|ccccc}
% \hline
% & ref. 0 & ref. 1 & ref. 2  \\\hline
% $y^+$ & 4.82 & 3.73 & 3.03 \\
% $N_{cells}/10^3$ & 170 & 197 & 223  \\
% \hline
% \end{tabular}
% \end{table}

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/naca_c_mesh_crop.png}
         \caption{full mesh}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/naca0012_mesh_close_coord.png}
         \caption{airfoil vicinity}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.9\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/naca0012_mesh_spanwise_coord.png}
         \caption{top view of the airfoil surface mesh}
     \end{subfigure}
        \caption{Various views of the computational mesh employed in the three-dimensional simulation.}
        \label{fig:mesh}
\end{figure}

Since the convective transport step is solved explicitly, the Courant number is limited to $\mathrm{Co}_{\mathrm{max}}=0.25$.
For larger values in the range $0.3 < \mathrm{Co} < 1$, the numerical solution is stable but yields spurious pressure values about the leading edge.
The dimensionless time step employed in the simulations is $\Delta \tilde{t}_{\mathrm{sim}}\approx 10^{-5}$, where the dimensionless time is defined as:
\begin{equation}
    \tilde{t} = \frac{ta_\infty}{c} = \frac{tU_\infty}{c\textrm{Ma}_\infty}\ ,
\end{equation}
and $a_\infty$, $U_\infty$, and $\mathrm{Ma}_\infty$ are the freestream speed of sound, velocity, and Mach number, respectively.
All simulations are conducted at $\mathrm{Re} = U_\infty c/\nu = 10^7$ and $\textrm{Ma} = U_\infty/a_\infty = 0.75$.

\subsection{Validation}

% validation from conference article
This section provides an excerpt of the more extensive validation procedure presented in Weiner and Semaan \cite{weiner2022}.
The validation mainly relies on experimental data from McDevitt and Okuno \cite{mcdevitt1985}.
% For the pre-onset angle of attack, $\alpha = 2^\circ$, experimental data by McDevitt and Okuno \cite{mcdevitt1985} is available for the local pressure coefficient $c_p$.
Figure \ref{fig:mesh_dep} shows a comparison between experimental and numerical pressure coefficient $c_p$ distributions at a pre-onset angle of attack of $\alpha = 2^\circ$.
% The numerical results were obtained with the 2D meshes.
In the figure, $\tilde{x}=x/c$ is a non-dimensionalized coordinate.
Similar normalization is applied to the other coordinates yielding $\tilde{y}$ and $\tilde{z}$.
As the figure shows, the numerical and experimental distributions compare favorably. 
We note the discrepancy in the shock location,
which is predicted approximately $0.05c$ upstream compared to the experiment.

\begin{figure}[t]
\centering
\includegraphics[width=0.75\textwidth]{figures/set1_cp_a2_iddes_refinement.pdf}
\caption{Comparison between the numerical and experimental pressure coefficient distributions of the NACA-0012 at $\alpha=2^\circ$ and $\textrm{Ma}_\infty=0.75$. The experimental data is from McDevitt and Okuno \cite{mcdevitt1985}.}
\label{fig:mesh_dep}
\end{figure}

At buffet conditions of $\alpha = 4^\circ$, a comparison of the pressure coefficient distribution is not possible, because of the lack of reference experimental data.
Therefore, we rely on the buffet frequency to validate the simulation results at these conditions.
Our results yield a buffet frequency of $\tilde{f}_b = \frac{2\pi c f}{U_\infty} \approx 0.65$ compared to $\tilde{f}_b=0.47$ from the experiment.
This discrepancy is within the expected range of numerically-obtained results from the literature considering that no additional tuning of turbulence model parameters was conducted \cite{iovnovich2012,weiner2022,kou2017}.

% Figure \ref{fig:a4_ref} shows the mean pressure coefficient and its temporal standard deviation for buffet conditions, $\alpha = 4^\circ$.
% The numerical results were again obtained with the 2D setup.
% No experimental reference data is available for comparison, but the results obtained on the three different refinement levels show very little mesh dependency both in the mean pressure coefficient and its standard deviation.
% Therefore, we believe the setup to be of sufficient quality for data generation and further analyses.

% \begin{figure}[hbt!]
% \centering
% \includegraphics[width=0.75\textwidth]{figures/set1_cp_a4_iddes_refinement.pdf}
% \caption{Pressure coefficient $c_p$ at $\alpha=4^\circ$ for several mesh resolutions according to table \ref{tab:meshes}; the shaded areas correspond to the standard deviation.}
% \label{fig:a4_ref}
% \end{figure}


\subsection{Data acquisition}

% data acquisition
Because we are interested in the transonic buffet dynamics,
all results presented in section \ref{sec:results} are based on the simulation at $\alpha = 4^\circ$.
Snapshots of density, velocity, pressure, and local Mach number are saved at an interval of $\Delta \tilde{t}\approx 5.5\times 10^{-2}$.
The time window used for the analysis, excluding the initial numerical transient, spans over $\Delta\tilde{T}_\mathrm{win}\approx 64$ corresponding to 5 full buffet cycles.
Consequently, about 230 snapshots per cycle are available.
This very high sampling rate is chosen with the intention to analyze the influence of the sampling rate on the DMD spectrum.

% slice and surface data, masking
To illustrate various scenarios, we analyze three different types of data: (i) surface pressure, (ii) a slice from the $\tilde{x}$-$\tilde{y}$-plane at $\tilde{z}=0$, and (iii) volume data.
For the surface data, we only consider the pressure on the upper surface, since tests including both upper and lower surfaces did not yield any significant differences.
For both the slice and volume data, only a subdomain spanning $-1 \le \tilde{x} \le 4$ and $-1 \le \tilde{y} \le 1$ is retained.
This masking operation reduces the overall data size and excludes unconverged downstream-convected structures from the analysis.
For brevity, we only present results from a data slice.
Results from the surface pressure and the volume data are provided in the repository.



==> nomenclature_old.tex <==
\section*{Nomenclature}

{\renewcommand\arraystretch{1.0}
\noindent\begin{longtable*}{@{}l @{\quad=\quad} l@{}}
$a$ & local speed of sound \\
$a_\infty$ & freestream speed of sound \\
$\mathbf{A}$ & discrete linear operator \\
$\mathbf{\mathcal{A}}$ & continuous linear operator \\
$\tilde{\mathbf{A}}$ & reduced discrete linear operator \\
$\mathbf{b}$ & DMD mode amplitudes \\
$c$ & chord length \\
$c_l$ & lift coefficient \\
$c_p$ & pressure coefficient \\
$Co$ & Courant number \\
$\mathbf{D}_\mathbf{b}$ & diagonal matrix based on $\mathbf{b}$ \\
$e$ & total energy density \\
$f$ & frequency \\
$f_b$ & buffet frequency \\
$f_s$ & snapshot sampling frequency \\
$\tilde{f}$ & normalized frequency \\
$I_i$ & importance of mode $i$ \\
$k$ & kinematic energy density \\
$\mathbf{L}$ & low-rank contributions to $\mathbf{M}$ \\
$\mathbf{M}$ & data matrix containing all snapshots \\
$\mathrm{Ma}$ & local Mach number \\
$\mathrm{Ma}_\infty$ & freestream Mach number \\
$N$ & number of snapshots \\
$N_{\mathrm{cells}}$ & number of control volumes \\
$N_{\mathrm{cycle}}$ & number of buffet cycles \\
$r$ & matrix rank \\
$r_{\mathrm{opt}}$ & optimal matrix rank \\
$Re_\infty$ & freestream Reynolds number \\
$\mathbf{S}$ & sparse contributions to $\mathbf{M}$ \\
$t$ & time \\
$\tilde{t}$ & normalized time \\
$\hat{u}$ & internal energy density \\
$\mathbf{u}$ & velocity vector \\
$u_\tau$ & friction velocity \\
$\mathbf{U}$ & matrix of left singular vectors \\
$U_\infty$ & freestream velocity \\
$\mathbf{V}$ & matrix of right singular vectors \\
$\mathbf{V}_\mathbf{\omega}$ & Vandermode matrix based on $\mathbf{\omega}$ \\
$w$ & weighting factor based on cell geometry \\
$\mathbf{W}$ & matrix of eigenvectors of $\tilde{\mathbf{A}}$ \\
$\tilde{x}$ & $x$-coordinate divided by chord length \\
$\mathbf{x}_n$ & snapshot of state vector at time step $n$ \\
$\mathbf{X}$ & data matrix of all but the last snapshots \\
$\mathbf{X}_r$ & truncated generic matrix $\mathbf{X}$ \\
$\tilde{y}$ & $y$-coordinate divided by chord length \\
$y^+$ & normalized coordinate normal to surface \\
$\mathbf{Y}$ & data matrix with all but the first snapshots \\
$\alpha$ & angle of attack \\
$\gamma$ & heat capacity ratio \\
$\gamma_0$ & sparsity control parameter in the spDMD \\
$\Delta t$ & time step \\
$\Delta\mathbf{X}$ & error in $\mathbf{X}$ \\
$\Delta\mathbf{Y}$ & error in $\mathbf{Y}$ \\
$\lambda$ & eigenvalue of $\mathbf{A}$ \\
$\lambda_0$ & sparsity control parameter in the robust SVD \\
$\mathbf{\Lambda}$ & matrix of eigenvalues of $\mathbf{A}$ \\
$\mu_x$ & temporal mean of generic $x$ \\
$\rho$ & density \\
$\sigma$ & singular value \\
$\sigma_x$ & temporal standard deviation of generic $x$ \\
$\mathbf{\Sigma}$ & matrix of singular values \\
$\tilde{\tau}$ & normalized correlation time lag \\
$\nu$ & kinematic viscosity \\
$\phi$ & DMD phase angle \\
$\mathbf{\Phi}$ & DMD modes, eigenvectors of $\mathbf{A}$ \\
$\mathbf{\Phi}_\mathbf{b}$ & $\mathbf{\Phi}$ with columns normalized by $\mathbf{b}$ \\
$\mathbf{\omega}$ & trace of $\mathbf{\Omega}$ \\
$\mathbf{\Omega}$ & matrix of eigenvalues of $\mathbf{\mathcal{A}}$ \\
$\Omega$ & domain \\
DES & Detached Eddy Simulation \\
DDES & Delayed DES \\
DMD & Dynamic Mode Decomposition \\
IDDES & Improved DDES \\
iPSP & instationary Pressure Sensitive Paint \\
LES & Large Eddy Simulation \\
mrDMD & multi resolution DMD \\
PIV & Particle Image Velocimetry \\
POD & Proper Orthogonal Decomposition \\
PSD & Power Spectral Density \\
SA & Spalart-Allmaras \\
SST & Shear Stress Transport \\
SVD & Singular Value Decomposition \\
spDMD & sparsity-promoting DMD \\
TDMD & Total least-squares DMD \\
RANS & Reynolds Averaged Navier Stokes \\
UDMD & Unitary DMD \\
URANS & Unsteady RANS \\
ZDES & Zonal DES \\
\end{longtable*}}

==> sampling_length_sensitivity.tex <==
As a final test, we examine DMD's sensitivity to the time window selection, which consists of sensitivity to the starting time and the time window length.
These tests are particularly relevant to numerical simulations, where the user has to decide when and how long to sample. 

For the starting time analysis, we apply DMD on a series of sequentially-shifted sequences, each sequence being shifted by a small time step.
We have tested three different time window lengths spanning between two and four buffet cycles.
In figure \ref{fig:sprectrum_time_window}, we present the results for three buffet cycles long sequence.
The spectra are visualized analogously to the ones in section \ref{sec:rank_sensitivity}, but with the abscissa now showing the starting time $\tilde{t}_0$ instead of the rank.
All spectra are computed on a planar slice through the flow field using optimal DMD.
The marker size in the figure is scaled by $I_i$ using the integral criterion, and the top ten markers are colored in red.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/f_bin_3cycles_uxya_r50.png}
    \caption{Opt. DMD spectra for a shifting time window of constant size covering three buffet cycles. The marker size is scaled by $I_i$ (integral criterion) and the top ten markers are colored in red. The state vector is the stagnation energy-conserving definition in equation \eqref{eq:final_state}.}
    \label{fig:sprectrum_time_window}
\end{figure}

As figure \ref{fig:sprectrum_time_window} shows, the starting time has little impact on the DMD spectrum.
Most relevant frequencies, including the high frequencies, remain consistent during the time shift.
We note that a perfectly non-varying spectrum with constant top frequencies over a shifting $\tilde{t}_0$ is not expected, because the IDDES simulation at this Reynolds number yields buffet cycle-to-cycle variations.
On the other hand, more consistent spectra can be expected with URANS data, because of its more regular time sequences.

For an appropriate rank selection and state vector definition, such as the one used in figure \ref{fig:sprectrum_time_window}, the DMD results are also insensitive to the time window length. 
%We note the shortest tested time window of two cycles, which we deliberately choose to ensure a minimal level of statistical convergence.
%Shorter sequences from this scale-resolving turbulent simulation risk yielding inconsistent results.
The low sensitivity to the total sampling time is in agreement with previously-reported DMD results from numerical and experimental investigations \cite{poplingher2019,ohmichi2018,masini2020}.
DMD spectra using other state vector definitions and rank truncations exhibit more variations (not shown) than what we observe in figure \ref{fig:sprectrum_time_window}.
More details are provided in the supplementary repository.
% The state vector based on the stagnation energy yields much more robust spectra for $\tilde{f}>2\tilde{f}_b$ compared to the other inner products.
% Stronger truncation of the POD basis clears up the spectra and reduces the variability of the dominant frequencies.
% Interestingly, the spectra of DMD and UDMD become more similar as the rank decreases, indicating that the default DMD operator becomes approximately unitary.
% However, if the POD basis is truncated too much, physically important structures with low energy content, like acoustic waves, are removed.
% More details about the sound waves follow in section \ref{sec:slice_analysis}.

In summary, for an appropriate rank and state vector definition, the choice of a time window has little influence on the DMD results.
We note that longer time sequences might be necessary if the cycle-to-cycle differences become stronger, which might be the case in experiments.

==> surface_volume_analysis.tex <==
To compare DMD results across different experimental or numerical data sources, it is important to assess if the same flow phenomena can be detected.
Therefore, we analyze surface and volume data in addition to the sample plane results presented in the previous section.

For the surface data, the state vector is based on the pressure coefficient $c_p$ on the upper surface. Using the full surface data yields almost identical results but introduces some additional visualization overhead.
Besides the changed state vector, the rest of the DMD workflow is exactly as described in the previous section.

The DMD spectrum resulting from the surface data is comparable to the one obtained from the sample plane; refer to the complementary material for a visualization.
Figure \ref{fig:dmd_modes_surface} shows the buffet mode and the most dominant vortex shedding mode.
Again, the buffet mode modifies the surface pressure about the shock and in the region of the separated boundary layer.
The phase-shifted combination of real and imaginary parts creates a periodic translatory motion of the pressure distribution along the chord.
The vortex shedding is characterized by fluctuations in the separated boundary layer, which display a significant variation along the chord and very little variation in spanwise direction.
There are also small ripples in the shock region, which are linked to the perturbation visible in figure \ref{fig:slice_dmd_phase} in the same range of $\tilde{x}$.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/naca_dmd_surface_modes_ref1.png}
    \caption{Selected DMD modes for $c_p$ on the wing section's upper surface.}
    \label{fig:dmd_modes_surface}
\end{figure}

To build the data matrix based on the volume data, only every fourth snapshot is used, resulting in a sampling frequency of $\tilde{f}_s/\tilde{f}_b \approx 58$.
As discussed in section \ref{sec:sampling_rate}, this sampling frequency can result in a mild truncation of frequencies at the upper end of the spectrum.
However, the memory requirement is greatly reduced and the resulting modes are qualitatively similar.
Besides the changed number of snapshots, the rest of the DMD workflow remains unchanged.

Figure \ref{fig:volume_mode} shows the most dominant mode in the vortex shedding region. The frequency is slightly lower than for the surface and slice data due to the reduced sampling rate.
Besides that, the mode's main features remain similar to the previous analyses.
The separated boundary layer and the detached vortices past the trailing edge are the most pronounced features.
Near the shock, the iso-contours capture some of the traveling sound waves.
Both the sound waves and the vortical structures show little variation in spanwise direction.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/vortex_shedding_mode.png}
    \caption{Iso-contours based on $\Re (a)$ for the DMD mode associated with vortex shedding at $\tilde{f}=10.05$ and upstream traveling waves.}
    \label{fig:volume_mode}
\end{figure}
